Front Transport Reduction for Complex Moving Fronts

This work addresses model order reduction for complex moving fronts, which are transported by advection or through a reaction-diffusion process. Such systems are especially challenging for model order reduction since the transport cannot be captured by linear reduction methods. Moreover, topological changes, such as splitting or merging of fronts pose difficulties for many nonlinear reduction methods and the small non-vanishing support of the underlying partial differential equations dynamics makes most nonlinear hyper-reduction methods infeasible. We propose a new decomposition method together with a hyper-reduction scheme that addresses these shortcomings. The decomposition uses a level-set function to parameterize the transport and a nonlinear activation function that captures the structure of the front. This approach is similar to autoencoder artificial neural networks, but additionally provides insights into the system, which can be used for efficient reduced order models. We make use of this property and are thus able to solve the advection equation with the same complexity as the POD-Galerkin approach while obtaining errors of less than one percent for representative examples. Furthermore, we outline a special hyper-reduction method for more complicated advection-reaction-diffusion systems. The capability of the approach is illustrated by various numerical examples in one and two spatial dimensions, including real-life applications to a two-dimensional Bunsen flame.

==> commands.tex <==
% ############################################################################
% 	My math shortcuts
% ############################################################################
\RequirePackage{amsmath}
%#####################
% 1. Model reduction
%####################
% singular value functional
\newcommand{\Jsigma}{\mathcal{J}}
\newcommand{\FTRmodes}{\matr{\Psi}}

%#####################
% 1. Physics
%####################
% singular value functional
\newcommand{\reactconst}{\gamma}
\newcommand{\diffconst}{\kappa}



%####################
% 2. General Math
%####################
\newcommand{\defeq}{\coloneqq}
\newcommand{\matr}[1]{\mathbf{#1}}
\newcommand{\tran}[1]{#1^{\intercal}}
\newcommand{\abs}[1]{\left | #1 \right |}
\newcommand{\ord}[1]{\mathcal{O}\left( #1 \right) }
\newcommand{\tr}[1]{\mathrm{tr}\left( #1 \right) }
\renewcommand{\vec}[1]{\boldsymbol{#1}}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
% Derivatives
\newcommand{\pd}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\td}[2]{\frac{\mathrm{d} #1}{\mathrm{d} #2}}
\renewcommand{\d}[1]{\mathrm{d}#1\;}
% Lp spaces:
\newcommand{\sprod}[2]{\langle #1 , #2 \rangle}
\newcommand{\norm}[1]{\Vert #1 \Vert}
\newcommand{\sigmoid}{\mathrm{sigmoid}}
% Linear algebra
\renewcommand{\u}{\vec{u}}
\newcommand{\Jmax}{\ensuremath{J_\mathrm{max}}}
\newcommand{\Jmin}{\ensuremath{J_\mathrm{min}}}
\newcommand{\Bs}{\ensuremath{B}}
\newcommand{\Grid}{\ensuremath{\Omega}}
\newcommand{\Block}{\ensuremath{\mathcal{B}}}
\newcommand{\Forest}{\ensuremath{\mathcal{F}}}
\newcommand{\err}{\ensuremath{\mathcal{E}}}
\newcommand{\errPOD}{\err_\text{POD}}
\newcommand{\smoothness}{\lambda_\text{smooth}}
\newcommand{\errWPOD}{\err_\text{wPOD}}
\newcommand{\errWavelet}{\err_\text{wavelet}}
\newcommand{\Tree}{\ensuremath{\mathcal{T}}}
\newcommand{\NTree}{\ensuremath{N_\mathrm{tree}}}
\newcommand{\NSnapshots}{\ensuremath{N_\mathrm{s}}}
\newcommand{\domain}{\Omega}
\newcommand{\Mode}{\vec{\Psi}}
\newcommand{\CompConst}{\mathcal{C}}
\newcommand{\Softwarename}[1]{\texttt{#1}}
\DeclareMathOperator{\curl}{\operatorname{curl}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\tikzpath}{figures/tikz}            %graphicspath to tikz pics
\newcommand{\highlight}[1]{{\color{blue}#1}}
\newcommand{\highlightKS}[1]{{\color{magenta}#1}}
\newcommand{\Smat}{\mathbf{U}}
\newcommand{\ucoef}{\underline{{\mathsf{u}}}}
\newcommand{\vcoef}{\underline{\boldsymbol{\mathsf{v}}}}
\newcommand{\kalpha}{\highlight{k_{{\alpha}}}}
\newcommand{\xalpha}{\highlight{x_{{\alpha}}}}


\newcommand{\Ntime}{N_t}
\newcommand{\define}[1]{\textit{#1}}
\newcommand{\sig}{\mathrm{sigmoid}}





%####################
% 3. Other
%####################
\newcommand{\todo}[1]{\textbf{\color{blue}#1}}
\newcommand{\philipp}[1]{{\color{blue}#1}}
\newcommand{\steffen}[1]{{\color{green!60!black}#1}}
\newcommand{\julius}[1]{{\color{orange!60!black}#1}}
\newcommand{\email}[1]{\href{mailto:#1}{#1}}
\newtheorem{problem}{Problem}


==> opti.tex <==
\section{FTR Optimization Problem}
For a given Snapshotmatrix $Q\in \mathbb{R}^{N_x,N_t}$ and front shape function $f\colon\mathbb{R}\to\mathbb{R}$ solve:
  \begin{align}
    \label{eq:OptimizationProblemFTR}
    \min_{\Phi\in\mathbb{R}^{N_x,N_t}} \Vert \Phi \Vert_* &+ \frac{\lambda}{2} \Vert D\Phi \Vert_\mathrm{F}^2\\
    \text{subject to}\quad & Q = f(\Phi)\,.
  \end{align}
  Here $[D_{ij}  = 1/2(\delta_{i,j-1}-\delta_{i,j+1})]_{i,j=1,\dots,N_x}$ a discrete differential operator acting on the columns of $\Phi$,
   $\|\cdot\|_{*}$ is the nuclear norm and
   $\|\cdot\|^2_{\mathrm{F}}$ the Frobenius norm.
   

\subsection{General Augmented Lagrangian Multiplier Method}

Convex high dimensional, non-smooth optimization problem, with constraints	\cite{LinChenMa2010,LinLiuSu2011}:
\begin{align*}
  \min g(X), \quad
  \text{subject to} \quad h(X) = 0
\end{align*}
Augmented Lagrangian Multiplier \cite{Hestenes1969}:
  \begin{equation}
    \mathcal{L}(X,Y) = g(X) + \langle Y,h(X) \rangle + \frac{\mu}{2}\Vert h(X) \Vert^2  _\mathrm{F}
  \end{equation}

  \includegraphics[width=1\linewidth]{augmentedlagrangianmultiplier.png}


\subsection{Augmented Lagrangian and Derivation of Algorithm}

To apply the general method of augmented Lagrange Multiplier to the FTR optimization problem \cref{eq:OptimizationProblemFTR} we identify $g(\Phi)=\norm{\Phi}_* + \lambda/2 \norm{D\Phi}_F^2$ and $h(\phi) = Q-f(\Phi)$. This yields the augmented Lagrangian with multiplier $Y$:
\begin{align*}
  \mathcal{L}(\Phi,Y,\mu)  = & \Vert \Phi \Vert_* + \frac{\lambda}{2} \Vert D\Phi\Vert^2  _\mathrm{F}  + \frac{\mu}{2}\Vert Q - f(\Phi)\Vert^2_\mathrm{F} \\
                       &+ \langle Y,Q - f(\Phi) \rangle 
\end{align*}
 $\argmin_\Phi   \mathcal{L}(\Phi,Y, \mu)$
  \begin{align*}
    \Rightarrow     &\quad\frac{\delta}{\delta \Phi}  \mathcal{L}(\Phi,Y)=0\\
    \Leftrightarrow &\quad\lambda D^*D\tilde{\Phi} - f'(\tilde{\Phi})[\mu(Q-f(\tilde{\Phi}))+Y] =0\\
    \text{and} &\quad\Phi =\operatorname{svt}(\tilde\Phi,\tau), \;\tau=1
  \end{align*}

  Soft thresholding SVD
  \begin{align*}
    \operatorname{svt}(\tilde\Phi,\tau) &= U \mathcal{S}_\tau (\Sigma) V^*\\
    &= \argmin_{\Phi}\tau\Vert \Phi \Vert_* + \frac{1}{2}\Vert \Phi - \tilde \Phi\Vert_F^2\\
    \mathcal{S}_\tau (x)&= \operatorname{sign}(x)\max(\abs{x}-\tau,0)
  \end{align*}

  \begin{figure}
    \centering
  \begin{tikzpicture}[scale=0.8]
      \draw[->] (-2,0) -- (-0.5,0) node[below] {$-\tau$} -- (0.4,0) node[below] {$\phantom{-}\tau$}
      -- (2,0) node[right] {$x$};
      \draw[->] (0,-1.2) -- (0,1.2) node[above] {$\mathcal{S}_\tau(x)$};
      \draw[scale=0.5,domain=-3:3,smooth,variable=\x,blue] plot ({\x},{sign(\x)*max(sqrt(\x*\x)-1,0)});
    \end{tikzpicture}
  \caption{Soft thresholding operator for thresholding singular values}
  \label{}
\end{figure}

\begin{algorithm}[H]
\caption{Alternating Direction Method for FTR}
\begin{algorithmic}[1]
\STATE $\Phi^0 = 0,Y^0=0$
\STATE $\epsilon_0 = \Vert Q-f(\Phi^0) \Vert_F$
\WHILE{$\epsilon_n > $err}
%\STATE {\color{black!60!white}($Y_{ij}^{n} = Y_{ij}^n-%\frac{1}{N_x}\sum_{k=1}^{N_x}Y_{kj}^n $)}
\STATE solve $D^*D \tilde \Phi^{n+1} = \frac{1}{\lambda}f'(\Phi^n)Y^n$
\STATE $\Phi^{n+1}=\operatorname{svt}(\tilde \Phi^{n+1},1)$
\STATE $Y^{n+1} =Y^{n} + \mu_n (Q-f(\Phi^n))$
\STATE $\epsilon_n = \Vert Q-f(\Phi^n) \Vert_F$
\STATE $n \leftarrow n+ 1$
\ENDWHILE
\end{algorithmic}
\end{algorithm}

